PrefixRL: Optimization of Parallel Prefix Circuits using Deep Reinforcement Learning

In this work, we present a reinforcement learning (RL) based approach to designing parallel prefix circuits such as adders or priority encoders that are fundamental to high-performance digital design. Unlike prior methods, our approach designs solutions tabula rasa purely through learning with synthesis in the loop. We design a grid-based state-action representation and an RL environment for constructing legal prefix circuits. Deep Convolutional RL agents trained on this environment produce prefix adder circuits that Pareto-dominate existing baselines with up to 16.0% and 30.2% lower area for the same delay in the 32b and 64b settings respectively. We observe that agents trained with open-source synthesis tools and cell library can design adder circuits that achieve lower area and delay than commercial tool adders in an industrial cell library.

==> results.tex <==
% Table generated by Excel2LaTeX from sheet 'table'
\begin{table}[htbp]
  \centering
  \caption{Experimental results For 32B Adder Optimization}\label{tab:results}
    \begin{tabular}{c|cc|cc|c|cc}
    \hline
    Design & \multicolumn{2}{c|}{Analytical} & \multicolumn{2}{c|}{Physical} & w\textsubscript{delay} & \multicolumn{2}{c}{Steps} \\
\cline{2-5}\cline{7-8}        & Area & Delay & Area & Delay &     & Gen. & Learn \\
    \hline
    RL01 & 53 & 20.0 & 1.000 & 1.448 & 0.08 & 13  & 1.45M \\
    RL02 & 54 & 18.0 & 1.010 & 1.307 & 0.12 & 15  & 2.05M \\
    RL03 & 55 & 17.5 & 1.020 & 1.223 & 0.10 & 16  & 1.46M \\
    RL04 & 56 & 17.0 & 1.030 & 1.193 & 0.15 & 15  & 1.42M \\
    RL05 & 57 & 16.5 & 1.040 & 1.185 & 0.20 & 18  & 1.34M \\
    RL06 & 59 & 16.0 & 1.060 & 1.153 & 0.25 & 18  & 3.41M \\
    RL07 & 60 & 15.5 & 1.069 & 1.153 & 0.25 & 18  & 2.63M \\
    RL08 & 63 & 15.0 & 1.099 & 1.107 & 0.45 & 13  & 2.39M \\
    RL09 & 66 & 14.5 & 1.129 & 1.078 & 0.50 & 19  & 2.69M \\
    RL10 & 70 & 14.0 & 1.169 & 1.053 & 0.70 & 20  & 2.32M \\
    RL11 & 76 & 13.5 & 1.228 & 1.000 & 0.70 & 26  & 3.56M \\
    RL12 & 83 & 13.0 & 1.298 & 1.006 & 0.95 & 30  & 3.02M \\
    \hline
    SA01 & 53 & 20.5 & 1.000 & 1.460 & -   & -   & - \\
    SA02 & 54 & 18.5 & 1.010 & 1.368 & -   & -   & - \\
    SA03 & 57 & 17.0 & 1.040 & 1.221 & -   & -   & - \\
    SA04 & 65 & 15.5 & 1.119 & 1.126 & -   & -   & - \\
    SA05 & 73 & 14.5 & 1.199 & 1.099 & -   & -   & - \\
    SA06 & 94 & 13.0 & 1.407 & 1.002 & -   & -   & - \\
    \hline
    ES01 & 74 & 21.0 & 1.208 & 1.271 & -   & -   & - \\
    ES02 & 56 & 19.5 & 1.030 & 1.371 & -   & -   & - \\
    \hline
    Sklansky & 80  & 23.5 & 1.268 & 1.395 & -   & -   & - \\
    KoggeStone & 129 & 15.5 & 1.754 & 1.048 & -   & -   & - \\
    BrentKung & 57  & 23.0 & 1.040 & 1.578 & -   & -   & - \\
    \hline
    \hline
\multicolumn{8}{l}{RL* designs are generates from PrefixRL agents}\\
\multicolumn{8}{l}{ES* designs are obtained from Exhaustive Search (ES) with pruning\cite{roy2014towards}}\\
\multicolumn{8}{l}{SA* designs are obtained from Simulated Annealing (SA)\cite{moto2018prefix}}\\
\multicolumn{8}{l}{Sklanksy, KoggeStone and BrentKung are regular structures \cite{sklansky1960conditional, kogge1973a, brent1982a}}\\
\multicolumn{8}{l}{Physical metrics are normalized}\\
\multicolumn{8}{l}{Scalarization weight w\textsubscript{area}$ = 1-$w\textsubscript{delay}}\\
\end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> results_analytical.tex <==
% Table generated by Excel2LaTeX from sheet 'table'
\begin{table}[htbp]
  \centering
  \caption{Analytical metrics for 32b Adder Optimization}\label{tab:results_analytical}
    \begin{tabular}{c|cc|c|cc}
    \hline
    Design & Area & Delay & w\textsubscript{delay} & \multicolumn{2}{c}{Steps} \\
\cline{5-6}        &  &  &     & Gen. & Learn \\
    \hline
    RL01 & 53 & 20.0 & 0.08 & 13  & 1.45M \\
    RL02 & 54 & 18.0 & 0.12 & 15  & 2.05M \\
    RL03 & 55 & 17.5 & 0.10 & 16  & 1.46M \\
    RL04 & 56 & 17.0 & 0.15 & 15  & 1.42M \\
    RL05 & 57 & 16.5 & 0.20 & 18  & 1.34M \\
    RL06 & 59 & 16.0 & 0.25 & 18  & 3.41M \\
    RL07 & 60 & 15.5 & 0.25 & 18  & 2.63M \\
    RL08 & 63 & 15.0 & 0.45 & 13  & 2.39M \\
    RL09 & 66 & 14.5 & 0.50 & 19  & 2.69M \\
    RL10 & 70 & 14.0 & 0.70 & 20  & 2.32M \\
    RL11 & 76 & 13.5 & 0.70 & 26  & 3.56M \\
    RL12 & 83 & 13.0 & 0.95 & 30  & 3.02M \\
    \hline
    SA01 & 53 & 20.5 & -   & -   & - \\
    SA02 & 54 & 18.5 & -   & -   & - \\
    SA03 & 57 & 17.0 & -   & -   & - \\
    SA04 & 65 & 15.5 & -   & -   & - \\
    SA05 & 73 & 14.5 & -   & -   & - \\
    SA06 & 94 & 13.0 & -   & -   & - \\
    \hline
    ES01 & 74 & 21.0 & -   & -   & - \\
    ES02 & 56 & 19.5 & -   & -   & - \\
    \hline
    Sklansky \cite{sklansky1960conditional} & 80  & 23.5 & -   & -   & - \\
    KoggeStone \cite{kogge1973a} & 129 & 15.5 & -   & -   & - \\
    BrentKung \cite{brent1982a} & 57  & 23.0 & -   & -   & - \\
    \hline
    \hline
\multicolumn{6}{l}{RL*: Generated from PrefixRL agents}\\
\multicolumn{6}{l}{ES*: Exhaustive Search (ES) with pruning\cite{roy2014towards}}\\
\multicolumn{6}{l}{SA*: Simulated Annealing (SA)\cite{moto2018prefix}}\\
\multicolumn{6}{l}{Scalarization weight w\textsubscript{area}$ = 1-$w\textsubscript{delay}}\\
\end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> results_synthesized.tex <==
% Table generated by Excel2LaTeX from sheet 'table'
\begin{table}[htbp]
  \centering
  \caption{Synthesized metrics for 32B Adder Optimization}\label{tab:results_synthesized}
    \begin{tabular}{c|cc}
    \hline
    Design & Area & Delay \\
    \hline
    RL01 & 1.000 & 1.448 \\
    RL02 & 1.010 & 1.307 \\
    RL03 & 1.020 & 1.223 \\
    RL04 & 1.030 & 1.193 \\
    RL05 & 1.040 & 1.185 \\
    RL06 & 1.060 & 1.153 \\
    RL07 & 1.069 & 1.153 \\
    RL08 & 1.099 & 1.107 \\
    RL09 & 1.129 & 1.078 \\
    RL10 & 1.169 & 1.053 \\
    RL11 & 1.228 & 1.000 \\
    RL12 & 1.298 & 1.006 \\
    \hline
    SA01 & 1.000 & 1.460 \\
    SA02 & 1.010 & 1.368 \\
    SA03 & 1.040 & 1.221 \\
    SA04 & 1.119 & 1.126 \\
    SA05 & 1.199 & 1.099 \\
    SA06 & 1.407 & 1.002 \\
    \hline
    ES01 & 1.208 & 1.271 \\
    ES02 & 1.030 & 1.371 \\
    \hline
    Sklansky \cite{sklansky1960conditional} & 1.268 & 1.395 \\
    KoggeStone \cite{kogge1973a} & 1.754 & 1.048 \\
    BrentKung \cite{brent1982a} & 1.040 & 1.578 \\
    \hline
    \hline
\multicolumn{3}{l}{RL*: Generated from PrefixRL agents}\\
\multicolumn{3}{l}{ES*: Exhaustive Search (ES) with pruning\cite{roy2014towards}}\\
\multicolumn{3}{l}{SA*: Simulated Annealing (SA)\cite{moto2018prefix}}\\
\multicolumn{3}{l}{Synthesized area and delay metrics are normalized\textsuperscript{\ref{fn:technode}}}\\

\end{tabular}%
  \label{tab:addlabel}%
\end{table}%

